LONER: LiDAR Only Neural Representations for Real-Time SLAM

This paper proposes LONER, the first real-time LiDAR SLAM algorithm that uses a neural implicit scene representation. Existing implicit mapping methods for LiDAR show promising results in large-scale reconstruction, but either require groundtruth poses or run slower than real-time. In contrast, LONER uses LiDAR data to train an MLP to estimate a dense map in real-time, while simultaneously estimating the trajectory of the sensor. To achieve real-time performance, this paper proposes a novel information-theoretic loss function that accounts for the fact that different regions of the map may be learned to varying degrees throughout online training. The proposed method is evaluated qualitatively and quantitatively on two open-source datasets. This evaluation illustrates that the proposed loss function converges faster and leads to more accurate geometry reconstruction than other loss functions used in depth-supervised neural implicit frameworks. Finally, this paper shows that LONER estimates trajectories competitively with state-of-the-art LiDAR SLAM methods, while also producing dense maps competitive with existing real-time implicit mapping methods that use groundtruth poses.

==> bonus_tables.tex <==
%Best of 5 versions
\begin{table*}[]
    \centering
\caption{Trajectory tracking results on loss comparison study. All numbers are best of 5 runs.}
\begin{tabular}{l l | c c c | c c c | c c c | c c c}
&& \multicolumn{3}{c|}{\textbf{Canteen Day}} & \multicolumn{3}{c|}{\textbf{Garden Day}} & \multicolumn{3}{c}{\textbf{MCR Slow 01}}& \multicolumn{3}{c}{\textbf{Quad Easy}} \\
&& $t_{ATE}$ & $t_{rel}$ & $r_{rel}$ & $t_{ATE}$ & $t_{rel}$ & $r_{rel}$ & $t_{ATE}$ & $t_{rel}$ & $r_{rel}$ & $t_{ATE}$ & $t_{rel}$ & $r_{rel}$\\
\cline{2-14}
\multirow{4}{*}{\textbf{\textbf{Full}}}
&Depth Loss&0.096  &0.101  &1.023  &0.067  &0.070  &1.160  &0.036  &0.047  &0.962  &0.230  &0.112  &1.799  \\
&LOS Slow&0.098  &0.079  &1.040  &0.079  &0.063  &0.946  &0.046  &0.071  &1.268  &0.201  &0.100  &1.141  \\
&LOS Medium&0.061  &0.067  &1.081  &0.044  &0.061  &1.155  &0.026  &0.057  &1.279  &0.094  &0.082  &1.226  \\
&LOS Fast&0.062  &0.068  &1.091  &0.044  &0.061  &1.150  &0.026  &0.055  &1.353  &0.094  &0.080  &1.230  \\
\cline{2-14}
&JS (Proposed)&0.062  &0.067  &1.085  &0.045  &0.060  &1.155  &0.026  &0.052  &1.260  &0.093  &0.083  &1.185  \\
\cline{2-14}
\multicolumn{1}{c}{\vspace{0.5cm}}\\
\cline{2-14}
\multirow{4}{*}{\textbf{\textbf{Lite}}}
&canteen &&& garden &&& mcr &&& quad\\
&Depth Loss&0.623  &0.096  &1.516  &0.430  &0.093  &1.566  &0.041  &0.061  &1.429  &0.949  &0.107  &1.814  \\
&LOS Slow&0.077  &0.081  &1.097  &0.112  &0.082  &1.277  &0.045  &0.072  &1.034  &0.271  &0.104  &1.458  \\
&LOS Medium&0.066  &0.073  &1.112  &0.062  &0.075  &1.086  &0.030  &0.058  &1.061  &0.174  &0.088  &1.212  \\
&LOS Fast&0.064  &0.073  &1.089  &0.056  &0.071  &1.097  &0.029  &0.061  &1.265  &0.177  &0.087  &1.205  \\
\cline{2-14}
&JS (Proposed)&0.064  &0.072  &1.209  &0.055  &0.075  &1.288  &0.030  &0.068  &1.244  &0.154  &0.099  &1.329  \\ 
\end{tabular}

\end{table*}


% best of 5 traj comparison
\begin{table*}[]
    \centering
\caption{Trajectory tracking results on SLAM ablation study. $t_{ATE}$ is RMSE ATE (m), $t_{rel}$ is RMSE 3m relative translation error, and $r_{rel}$ is RMSE 3m relative rotation error (deg). All numbers are best of 5 runs.}
\begin{tabular}{l l | c c c | c c c | c c c | c c c}
&& \multicolumn{3}{c|}{\textbf{Canteen Day}} & \multicolumn{3}{c|}{\textbf{Garden Day}} & \multicolumn{3}{c}{\textbf{MCR Slow 01}}& \multicolumn{3}{c}{\textbf{Quad Easy}}  \\
&& $t_{ATE}$ & $t_{rel}$ & $r_{rel}$ & $t_{ATE}$ & $t_{rel}$ & $r_{rel}$ & $t_{ATE}$ & $t_{rel}$ & $r_{rel}$& $t_{ATE}$ & $t_{rel}$ & $r_{rel}$\\
\cline{2-14}
\multirow{5}{*}{\textbf{\textbf{Full}}}
&No Pose Opt.&1.060  &0.067  &1.317  &1.256  &0.064  &1.273  &0.081  &0.065  &1.605  &0.583  &0.079  &1.267  \\
&No Motion Comp.&0.065  &0.071  &1.143  &0.046  &0.058  &0.992  &0.028  &0.051  &1.334  &0.094  &0.081  &1.130  \\
&Random KFs&0.061  &0.064  &1.034  &0.045  &0.060  &1.157  &0.027  &0.050  &1.263  &0.089  &0.082  &1.220  \\
&Temporal KFs&0.062  &0.066  &1.080  &0.047  &0.061  &1.146  &0.027  &0.051  &1.415  &0.222  &0.082  &1.177  \\
\cline{2-14}
&Proposed&0.062  &0.067  &1.085  &0.045  &0.060  &1.155  &0.026  &0.052  &1.260  &0.093  &0.083  &1.185  \\
\cline{2-14}

\multicolumn{1}{c}{\vspace{0.5cm}}\\

\cline{2-14}
\multirow{5}{*}{\textbf{\textbf{Lite}}}
&No Pose Opt.&1.083  &0.069  &1.265  &1.119  &0.061  &1.338  &0.088  &0.060  &1.535  &0.903  &0.084  &1.253  &\\
&No Motion Comp.&0.062  &0.072  &1.219  &0.060  &0.073  &1.084  &0.030  &0.056  &1.591  &0.129  &0.096  &1.236  \\
&Random KFs&0.063  &0.071  &1.067  &0.056  &0.072  &1.130  &0.029  &0.067  &1.250  &0.113  &0.086  &1.265  \\
&Temporal KFs&0.083  &0.070  &1.134  &0.066  &0.071  &1.130  &0.029  &0.067  &1.248  &0.246  &0.087  &1.249  \\
\cline{2-14}
&Proposed&0.064  &0.072  &1.209  &0.055  &0.075  &1.288  &0.030  &0.068  &1.244  &0.154  &0.099  &1.329  \\
\cline{2-14}

\end{tabular}
\end{table*}


% Median of 5 AREs: Full Traj Comparison
\begin{table*}
\begin{tabular}{l |c c c c}
No Pose Opt.&5.493  &5.647  &7.085  &2.031  \\
No Motion Comp.&0.917  &0.956  &6.937  &1.220  \\
Random KFs&0.864  &1.003  &6.955  &1.219  \\
Temporal KFs&0.879  &0.996  &6.960  &1.302  \\
Proposed&0.864  &1.001  &6.959  &1.217  \\
\end{tabular}
\end{table*}



% Median of 5 AREs: Full Map Comparison
\begin{table*}
\begin{tabular}{l |c c c c}
&canteen & garden & mcr & quad\\
Depth Loss&0.924  &1.063  &6.998  &1.728  \\
LOS Slow&0.853  &1.014  &6.959  &1.287  \\
LOS Medium&0.866  &1.006  &6.958  &1.222  \\
LOS Fast&0.865  &1.001  &6.960  &1.221  \\
Proposed&0.864  &1.001  &6.959  &1.217  \\
\end{tabular}
\end{table*}



% Best of 5 AREs: Lite Traj Comparison
\begin{table*}
\begin{tabular}{l |c c c c}
&canteen & garden & mcr & quad\\
No Pose Opt.&5.826  &4.916  &7.155  &2.722  \\
No Motion Comp.&0.930  &1.062  &6.932  &1.304  \\
Random KFs&0.896  &1.119  &6.956  &1.221  \\
Temporal KFs&0.962  &1.119  &6.951  &1.258  \\
Proposed&0.900  &1.119  &6.956  &1.262  \\
\end{tabular}
\end{table*}


% Best of 5 AREs: Lite Map Comparison
\begin{table*}
\begin{tabular}{l |c c c c}
&canteen & garden & mcr & quad\\
Depth Loss&3.170  &2.510  &6.948  &2.628  \\
LOS Slow&0.925  &1.140  &6.959  &1.325  \\
LOS Medium&0.899  &1.106  &6.954  &1.305  \\
LOS Fast&0.904  &1.105  &6.952  &1.290  \\
Proposed&0.900  &1.119  &6.956  &1.262  \\
\end{tabular}
\end{table*}



\begin{table*}  \label{tracking}
\begin{center}
\begin{tabular}{l | c  c  c | c c c }
\hline
& LiDAR & Stereo & IMU & Canteen Day & Garden Day & MCR Slow 01 \\
\hline
\textbf{VINS-Fusion} & \xmark & \cmark & \cmark & 0.691 & 0.518 & 0.081 \\
\textbf{LIO-SAM} & \cmark & \xmark & \cmark & \textbf{0.053} & 0.069 & \textbf{0.030} \\
\hline
\textbf{\algname} & \cmark & \xmark & \xmark & 0.068 &\textbf{0.058} &0.037  \\
\textbf{\algname lite} & \cmark & \xmark & \xmark & 0.076  &0.061 &0.031   \\
\hline
\end{tabular}
\end{center}
\caption{Pose tracking results on Fusion Portable sequences. $t_{ATE}$ is RMSE ATE (m), $t_{rel}$ is RMSE 1m relative translation error, and $r_{rel}$ is RMSE 1m relative rotation error (deg). All numbers are a median of 10 runs.}
\end{table*}




\begin{table}[]
    \centering
\begin{tabular}{l | c c c }
& $t_{ATE}$ & $t_{rel}$ & $r_{rel}$\\
\hline
{VINS-Fusion} & 0.691 & 0.518 & 0.081 \\
{LIO-SAM} & 0.053 & 0.069 & 0.030 \\
\hline
{Fast Epsilon Decay} &0.070  &0.021  &0.259  \\
{Slow Epsilon Decay} &0.101  &0.067  &0.592  \\
{With JS Loss} &0.069 &0.067  &0.592
\end{tabular}
\caption{Comparison of Trajectory Accuracy with and without JS Loss. $t_{ATE}$ is RMSE ATE (m), $t_{rel}$ is RMSE Rel Err (m/m), $r_{rel}$ is RMSE Rel Rot. Err (deg/m). Results are a median of 10 runs on the Canteen Day sequence.}
\end{table}


\begin{table*}  \label{tracking}
\begin{center}
\begin{tabular}{l | c c c }
\hline
& Canteen Day & Garden Day & MCR Slow 01 \\
\hline
\textbf{VINS-Fusion} & 0.691 & 0.518 & 0.081 \\
\textbf{LIO-SAM} & \textbf{0.053} & 0.069 & \textbf{0.030} \\
\hline
\textbf{\algname} & 0.068 &\textbf{0.058} &0.037  \\
\textbf{\algname lite} & 0.076  &0.061 &0.031   \\
\hline
\end{tabular}
\end{center}
\caption{Pose tracking results on Fusion Portable sequences. $t_{ATE}$ is RMSE ATE (m), $t_{rel}$ is RMSE 1m relative translation error, and $r_{rel}$ is RMSE 1m relative rotation error (deg). All numbers are a median of 10 runs.}
\end{table*}



\begin{table} \label{traj-ablation}
    \centering
    \begin{tabular}{l | c c c | c }
    \hline
    \multirow{2}{*}{Type} & \textbf{Pose} & \textbf{Random} & \textbf{Motion} & \textbf{RMSE} \\
    & \textbf{Opt.} & \textbf{Window} & \textbf{Comp.} & \textbf{ATE (m)}\\
    \hline
    \textbf{Ablation A} & \xmark & \cmark & \cmark & 0 \\
    \textbf{Ablation B} & \cmark & \xmark & \cmark & 0\\
    \textbf{Ablation C} & \cmark & \cmark & \xmark & 0\\
    \textbf{Ablation D} & \cmark & \cmark & \cmark & 0 \\
    \hline
    \textbf{Proposed} & \cmark & \cmark & \cmark & 0 \\
    \hline
    \end{tabular}
    \caption{Ablation study on trajectory accuracy. The full (not lite) model was used in each configuration.}
\end{table}

\begin{table*} \label{map-ablation}
    \centering
    \begin{tabular}{l | c c c c | c c c c}
    \hline
    \multirow{2}{*}{Type} & \textbf{Depth} & \textbf{LOS} & \textbf{JS} & \textbf{Decouple}  & \multirow{2}{*}{\textbf{Depth L1} $\downarrow$} & \multirow{2}{*}{\textbf{Acc.} $\downarrow$} & \multirow{2}{*}{\textbf{Comp.} $\downarrow$} & \textbf{Comp.} \\
    & \textbf{Loss} & \textbf{Loss} & \textbf{Loss} & \textbf{RGB/LiDAR} &&&&\textbf{Ratio $\uparrow$}\\
    \hline
    \textbf{Ablation A} & \cmark & \xmark & \xmark & \cmark & 0 & 0 & 0 & 0\\
    \textbf{Ablation B} & \xmark & \cmark & \xmark & \cmark & 0 & 0 & 0 & 0\\
    \textbf{Ablation C} & \xmark & \xmark & \cmark & \xmark & 0 & 0 & 0 & 0\\
    \hline
    \textbf{Proposed} & \xmark & \xmark & \xmark & \cmark & 0 & 0 & 0 & 0\\
    \hline
    \end{tabular}
    \caption{Ablation study on map accuracy. The full (not lite) model was used in each configuration. Ground truth poses were used for all experiments and pose optimization was disabled.}
\end{table*}


==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> response_to_reviewers/blankpage.tex <==
\;
\pagebreak

==> response_to_reviewers/editor.tex <==
\AEreview


==> response_to_reviewers/reviewer1.tex <==
\reviewer

\textit{The authors propose an innovative LiDAR SLAM using Neural representations, specifically designed to operate efficiently in outdoor environments. The authors introduce a novel loss function, which enables faster convergence compared to existing alternatives. Experimental results demonstrate improved accuracy in localization and mapping when employing the proposed loss function.}


\subsection*{Comments}

\comment{Compelling outcomes are presented, demonstrating that the proposed method outperforms traditional LiDAR SLAM and neural implicit RGBD SLAM in terms of pose estimation performance. Furthermore, the method exhibits superior mapping performance on real-world datasets when compared to other neural implicit representations for LiDAR sensors. The investigation into runtime performance reveals that the method can achieve a real-time online capability of 5Hz for LiDAR processing.}

\response{
We are grateful to the reviewer for their kind remarks about our paper.
}

\pagebreak

\comment{It would be interesting to witness the
presentation of results pertaining to a challenging dataset, such as scenarios that are repeated frequently and
characterized by a lack of diverse features.}


\response{
We appreciate this suggestion and agree that testing on more challenging datasets is an important avenue of investigation.

In the paper, we test on four datasets. The first is MCR: a small, indoor, feature-rich lab environment. Next, we test on Canteen and Garden, both semi-outdoor courtyard environments. MCR, Canteen, and Garden are all from the Fusion Portable dataset \cite{fusion-portable}. Additionally, we aimed to demonstrate performance in settings that are physically larger and where the LiDAR would see farther into the distance. While many datasets exist, we struggled to find one that provided data from a suitable LiDAR with corresponding ground-truth trajectory and map data for evaluation. In the end, we settled on the Quad sequence from the Newer College dataset \cite{newer-college}. The Quad environment is enclosed, but it is not as feature-rich as the other three datasets. While the walls are textured, they also form a pattern that is repeated relatively uniformly throughout the sequence. Further, the motion consists of two loops around the scene. We believe this demonstrates the ability of our system to work in more open, feature-sparse environments. 

Operating in very large environments (such as open roads), or in environments with extreme feature sparsity (such as fields and off-road environments) would be unlikely to perform well. Extreme feature sparsity makes tracking difficult since there are few distinguishing features in the environment, while large-scale environments such as open roads require the system to learn geometry faster than memory and compute constraints allow. However, we are actively working on addressing these areas, which will hopefully be the subject of future publications. Further, in the future, we will consider collecting our own datasets that help bridge the gap between what we have tested so far and these very large environments.

To provide an additional demonstration of our method for the reviewers, we have qualitatively evaluated LONER on datasets recorded during the DARPA subterranean challenge \cite{DARPA}, which exhibit some of the feature sparsity the reviewer expressed interest in seeing. These results will not fit in the page limit of the paper, but they have been added to the project webpage: \url{https://umautobots.github.io/loner}. 

}

\pagebreak
\comment{
The authors propose the incorporation of a dynamic margin loss, utilizing the Jensen-Shannon divergence, into the loss function to enhance the efficacy of the map refining strategy. However, I find Equation (7) and (8) somewhat perplexing. 
}


\response{

We thank the reviewer for their feedback. We've restructured the definition of the JS loss to reduce confusion. In summary, the primary component of the loss is the difference between the weight computed with the neural network (denoted $w_i$), and the target weight given by the truncated Gaussian $\mathcal{K}_\epsilon$ (denoted $w_i^*$). In the first draft, Equation 7 captured this primary loss: $\mathcal{L}_{sight}(\Theta) = \lVert w_i^* - w_i\rVert_1$. Additionally, we add a second mechanism to ensure that the weights sum to 1, and thus form a probability distribution. Following terminology used in \cite{cloner}, we denote this as the Opacity loss, which was formerly Equation 8: $\mathcal{L}_{opacity}(\Theta) = \lVert 1 - \sum_iw_i\rVert_1$. This opacity loss formulation was borrowed from CLONeR, which is work that preceded LONER \cite{cloner}. The change is summarized below:

\begin{center}
\textbf{Original:}

\setcounter{equation}{5}
\begin{align}
    % \begin{split} % This forces only one number for the entire block; get rid of it to have three separate equation numbers.
    \mathcal{L}_{JS}(\Theta) &= \mathcal{L}_{sight} + \mathcal{L}_{opacity} \\
    \mathcal{L}_{sight}(\Theta) &= \lVert w_i^* - w_i \rVert_1 \\
    \mathcal{L}_{opacity}(\Theta) &= \lVert 1 - \sum_i w_i \rVert_1
    % \end{split}
\end{align}

\textbf{Updated:}

\setcounter{equation}{5}
\begin{equation}
\mathcal{L}_{JS}(\Theta) =  \underbrace{\lVert w_i^* - w_i \rVert_1}_{\text{Primary Loss}}  + \underbrace{\lVert 1 - \sum_i w_i \rVert_1}_{\text{Opacity Loss}},
\end{equation}

    
\end{center}

Further, we have added a citation to CLONeR \cite{cloner} in the discussion of the loss, as CLONeR provides more details on the need for the Opacity loss:

\textit{...where the opacity loss \reviewadd{\it (explained in more detail by \cite{cloner})} ensures weights along each ray sum to one \reivewadd{thus forming a probability distribution}.}

}

\comment{
 And in the first paragraph of section III-E-1), $w_i$ is defined in equation 2. 
}

\response{
We have updated the reference to the definition of $w_i$ in the first paragraph of section III-E-1 to now correctly point to Equation 2 instead of Equation 1. 
}

\comment{
Additionally, it would be beneficial if the authors explicitly mentioned whether they utilize the IMU as an
initial guess for ICP
}

\response{
We added the following sentence to the System Overview section (Section III-A) to highlight that an IMU is not used to initialize ICP:

 \reviewadd{\it \algname is designed for use without an IMU, so ICP uses the identity transformation as an initial guess.}

Finally, we expanded the explanation in the conclusions section on why IMU integration may be an important avenue of future work:

{\it Further, inertial data could help the system track accurately under rapid rotation \reviewadd{\it and in feature-sparse scenarios, where the LiDAR data is less informative}}
}

==> response_to_reviewers/reviewer2.tex <==
\reviewer

\textit{The paper proposes a Lidar SLAM system which uses an implicit representation. The main contribution of the paper is the introduction of a dynamic threshold for the kernel in the Line of sight prior loss as opposed to existing methods which use a fixed threshold for all LIDAR rays. This allowed the system to be brought up to real-time performance while offering accurate pose estimation and 3D reconstruction.}


\subsection*{Comments}

\comment{
General remarks: 

\begin{itemize}
    \item The paper is well written and easy to understand.
    \item The use of a dynamic threshold per ray based on the JS metric makes sense.
    \item The remaining parts of the SLAM system (selection of keyframe, optimization heuristics) are well-described and seem to contribute to bringing the system to real-time performance.
    \item The algorithm is compared against state-of-the art algorithms and several ablation studies have been performed to verify the importance of each component of the proposed loss. 
\end{itemize}
}

\response{We thank the reviewer for their kind remarks about our paper.}

\comment{
Are the values of $JS_{max}$ and $JS_{min}$ heuristically tuned? 
}

\response{
We appreciate the reviewer's comments. We've updated the paper to address each of their concerns.

We added language to the Implementation Details section (Section IV-A) to indicate that all parameter values were tuned experimentally. While there is limited space in the paper for further discussion, we can provide more details here. 

In practice, we tune those parameters through exhaustive search experiments. We found setting $JS_{min}$ from 1 to 5, $JS_{max}$ from 10 to 15, and $\alpha$ from 1 to 5 provides good results, and variations within those ranges do not significantly impact performance. As a result, we simply selected the roundest values of $JS_{min} =1$, $JS_{max} =10$, and $\alpha = 1$.
}

\comment{
Did the parameter in table 1 offer good generalization across the datasets? 
}
\response{
Yes, all parameter values were tuned experimentally, and we found them to generalize well across the datasets. All experiment results shown in the paper are using the parameters in Table 1. We've added language to the Implementation Details section (Section IV-A) to clarify this.
}

\pagebreak
\comment{
In section IV.D, the authors state that “LONER using the URF loss is less competitive, indicating that the L2 LOS loss is not suitable for real-time SLAM”. The L2 loss seems to affect the accuracy but does it necessarily affect the real-time performance?   
}

\response{
The authors believe that the L2 loss performs poorly in our system because we run significantly fewer total iterations than Urban Radiance Fields (URF, \cite{urf}) does. Because the L2 loss weighs outliers heavily, we believe that few outliers can dominate the gradient early in training. In the context of an offline optimization, such as in URF, this is not a problem: eventually, the effect of outliers will be reduced and the gradient can focus on reconstructing the rest of the geometry. However, with the limited number of iterations we run to maintain real-time performance, we believe these outliers dominate training and as a result, the overall reconstruction is much worse. Hence, with unbounded iterations the L2 loss performs well, but in our real-time system the L1 loss appears to be significantly better. 

Because we cannot confirm this speculation, we've updated the sentence and only mentioned our observation:

\textit{We found LONER using the URF loss is less competitive\reviewremove{, {\it indicating that the L2 LOS loss is not suitable for real-time SLAM}.}}
}

==> response_to_reviewers/reviewer3.tex <==
\reviewer 

\textit{The paper presents a real-time neural implicit LiDAR SLAM with tracking done by point-to-plane ICP and mapping done with a NeRF-style MLP. To improve the convergence speed and reconstruction quality, a dynamic margin loss which is based on the Jasen-Shannon divergence is proposed. The proposed system indeed achieved better performance than RGB-D neural implicit SLAM and conventional LiDAR SLAM. }

\subsection*{Comments}


\comment{
Related works: there has been a booming development in NeRF-based SLAM, but Section II-B missed a big trunk of related works. Below are the already published related works. 

[1] E. Kruzhkov et al., "MeSLAM: Memory Efficient SLAM based on Neural Fields," 2022 IEEE International Conference on Systems, Man, and Cybernetics (SMC), Prague, Czech Republic, 2022, pp. 430-435. 

[2] X. Yang, H. Li, H. Zhai, Y. Ming, Y. Liu and G. Zhang, "Vox-Fusion: Dense Tracking and Mapping with Voxel-based Neural Implicit Representation," 2022 IEEE International Symposium on Mixed and Augmented Reality (ISMAR), Singapore, Singapore, 2022, pp. 499-507. 

[3] Hengyi Wang, Jingwen Wang and Lourdes Agapito, "Co-SLAM: Joint Coordinate and Sparse Parametric Encodings for Neural Real-Time SLAM," in 2023 IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR), 2023, pp. 13293-13302. 

[4] Mohammad Mahdi Johari, Camilla Carta and François Fleuret, "ESLAM: Efficient Dense SLAM System Based on Hybrid Representation of Signed Distance Fields," in 2023 IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR), 2023, pp. 17408-17419. 
}

\response{
We thank the reviewer for their suggestions. We have updated the paper to include these references. 
}

\pagebreak


\comment{
Keyframe selection criterion: the paper used the time passed as the criterion to select keyframes, which I believe is sub-optimal. If the sensor stays at the same position for a long time, or if the sensor moves in a loopy motion, it is very likely the same or similar keyframe will be kept adding to the system. 
}

\response{
We thank the reviewer for their suggestion. Throughout the development of LONER, the authors have considered ways to solve the suboptimality the reviewer noticed. Our extensive testing indicated that each KeyFrame should be processed for approximately three seconds before moving on, leading to the selection of $t_{KF} = 3$. Hence, even if significant motion is observed in those three seconds, there is no practical way to add a new KeyFrame and restart the optimization without sacrificing the convergence of the previous KeyFrame, which can affect overall accuracy. Three alternatives were considered.

First, after reading this reviewer's comment, we implemented a modification to \algname that monitors the frames processed by the tracker. If sufficient motion is detected, this monitoring thread interrupts the mapping optimization, adds a new KeyFrame, then restarts the optimizer. However, due to parallelism limitations in Python, we found this to introduce sufficient overhead such that it was not practical. Additionally, we struggled to guarantee that the previous KeyFrame's optimization had sufficiently converged before starting the next.

Next, we considered simply not adding a KeyFrame unless $t_{KF}$ has passed \textbf{and} some minimum motion criteria (either 0.5m of translation \textbf{or} 22.5$^\circ$ of rotation) has been met. If that motion condition is not met, then the mapper idles until both conditions are met. However, this leads the optimizer to run fewer overall iterations. Hence, this configuration generally led to degraded performance, as reported in Table \ref{tab:kf_ablation}. We report RMSE APE (median of five runs), as well as the L1 depth reconstruction error compared to \algname. This configuration is denoted ``Hybrid Lazy".

Finally, we implemented a slight variation of the above test. If after $t_{KF}$ the distance criterion was not met, then a new KeyFrame is not added, as above. However, rather than idling, the mapping process is then re-run with the existing set of KeyFrames. This addresses the reviewer's concerns about adding excess KeyFrames that are very close to each other, while also ensuring that the mapper runs as many total iterations as possible. As is reported in Table \ref{tab:kf_ablation}, this did not significantly change the result over the baseline algorithm. We believe this to reflect that having more diversity of data does not harm performance, even when the difference is minor. In Table \ref{tab:kf_ablation}, this configuration is denoted ``Hybrid Eager".

While the results of the above experiments will be omitted from the paper due to space limitations, we will include them in an appendix on the project webpage upon paper publication. 

In summary, we appreciate the reviewer's suggestion to consider alternate ways of adding KeyFrames. While we agree that there is room to improve on this in the future, on the datasets we tested on, we found that a temporal metric was the most practical. However, we agree with the reviewer that in some datasets that include lots of time at rest, one of these distance-based metrics may outperform the temporal metric. As a result, we will include settings to enable the ``Hybrid Eager" and ``Hybrid Lazy" configurations in the code release, along with documentation indicating when to use these options.
}


\input{tables/kf_ablation.tex}
\pagebreak

\comment{
When evaluating tracking performance, only RMS of APE is provided while in other nerf-SLAM papers, not only RMS but also mean and median are provided.
}

\response{
% iMAP -> ATE RSME
% nice slam -> ATE RSME best of 5 runs
% MeSLAM -> ATE RSME
% CoSLAM -> ATE RSME
% Vox-Fusion -> ATE RSME, Mean, Median
% ESLAM -> ATE RSME, Mean
We thank the reviewer for the suggestion. %Due to a lack of consistency across the implicit SLAM literature, our decision for formatting this trajectory data was made by deferring to ORB-SLAM \cite{orbslam}. 

We found a lack of consistency across the implicit SLAM literature, including previous works we compare against and works the reviewer recommends to cite. Most works such as iMAP, NICE-SLAM, MeSLAM, and CoSLAM only provide RMS ATE in the paper. Only Vox-Fusion and ESLAM provide mean errors, and Vox-Fusion is the only work that provides median errors. Due to this lack of consistency, our decision for data reporting was made by deferring to ORB-SLAM \cite{orbslam}.

We agree with the reviewer that including more data would be useful for some readers. However, due to space limitations, we cannot fit the data in a digestible way within the paper. Instead, we will include the complete data tables recommended by the reviewer in an appendix that will be posted to the project website upon paper acceptance. Finally, we will post the raw data tables to the website following acceptance of the paper. The following language has been added to the Implementation Details section (IV-A):

\reviewadd{\it The complete data from our evaluations is available on the project webpage.}

We hope this provides readers who want more detail with the opportunity to find it, without sacrificing the clarity of the paper. 
}

\pagebreak

\comment{
Regarding the tracking module, the paper directly adopted the point-to-plane ICP rather than inverse-NeRF style optimization. It would be interesting to see some discussions even ablation studies on why ICP is chosen over iNeRF optimization. 
}

\response{
We thank the reviewer for this suggestion. There are two reasons we chose to use ICP rather than iNeRF optimization.

First, ICP is a simple, fast, and reliable method for motion estimation. Thus, it is a practical choice for our system and we found it to provide very strong performance. While many NeRF-based SLAM papers use iNeRF, those systems are generally based on RGB or RGB-D sensors, for which direct solutions to motion estimation are either unavailable or less reliable than when using LiDAR. Further, ICP runs on the CPU while iNeRF optimization runs on the GPU. Since the GPU is the limiting resource in our system, we chose to limit the tracker to running on the CPU such that the mapper can occupy the entire GPU.

Second, we found that in our system the iNeRF optimization performs poorly. We ran internal tests where ICP is used first, followed by an iNeRF refinement, followed by a joint optimization. However, the iNeRF refinement step hurt performance. While we hope to determine why this happens in the future, due to the strong performance of ICP, fixing this issue was not a high priority. 

While a complete discussion of this cannot be fit within the paper, we added the following text to Section III.B to highlight this decision:

\reviewadd{\it We adopted ICP rather than inverse-NeRF due to strong performance and to save the GPU resources for the mapping module to maintain real-time performance.}
}

==> response_to_reviewers/tables/kf_ablation.tex <==

\begin{table}[hb!]
    \centering
    \caption{Comparison of three KeyFrame selection criteria. The first, Default, is the strategy implemented in the LONER paper which adds a new KeyFrame every time $t_{KF}$ has past (3s in default configuration). The second strategy is Hybrid Lazy, which waits until at least 3 seconds has passed and a minimum motion threshold of either 0.5m of translation or 22.5$^\circ$ of rotation is met. The third is Hybrid Eager, which combines the two: if after 3 seconds the motion criteria is not met, it does not add a new KeyFrame, but instead re-runs the optimization with the existing KeyFrames. }

    \begin{tabular}{l|c|c|c|c|c|c|c|c}
    &\multicolumn{2}{c|}{Canteen}&\multicolumn{2}{c|}{Garden}&\multicolumn{2}{c|}{MCR}&\multicolumn{2}{c}{Quad}	\\
    \hline
    & RMS&L1&RMS&L1&RMS&L1&RMS&L1\\
    & APE & Depth & APE & Depth & APE & Depth & APE & Depth\\
    \hline
    Default	      &0.063	&\textbf{1.354}	&\textbf{0.056}	&1.249	&\textbf{0.029}	&0.239	&0.127	&0.899 \\
    Hybrid Lazy	  &\textbf{0.062}	&1.417	&0.059	&1.314	&\textbf{0.029}	&0.240	&0.142	&1.030 \\
    Hybrid Eager	&\textbf{0.062}	&1.388	&0.062	&\textbf{1.224}	&\textbf{0.029}	&\textbf{0.231}	&\textbf{0.123}	&\textbf{0.847} \\
    \hline
        \end{tabular}
    \label{tab:kf_ablation}
\end{table}


==> tables/loss_comparison.tex <==

\begin{table*}
    \centering
\caption{Trajectory tracking results on loss comparison study. All numbers are a median of 5 runs.}
\label{loss-comparison}
\begin{tabular}{l l | c c c | c c c | c c c | c c c}
&& \multicolumn{3}{c|}{\textbf{Canteen Day}} & \multicolumn{3}{c|}{\textbf{Garden Day}} & \multicolumn{3}{c}{\textbf{MCR Slow 01}}& \multicolumn{3}{c}{\textbf{Quad Easy}} \\
&& $t_{ATE}$ & $t_{rel}$ & $r_{rel}$ & $t_{ATE}$ & $t_{rel}$ & $r_{rel}$ & $t_{ATE}$ & $t_{rel}$ & $r_{rel}$ & $t_{ATE}$ & $t_{rel}$ & $r_{rel}$\\
\cline{2-14}
\multirow{4}{*}{\textbf{\textbf{Full}}}
&Depth Loss &0.160 &0.108 &1.241 &0.083 &0.074 &1.330 &0.045 &$\mathbf{0.054}$ &1.155 &0.303 &0.124 &1.899 \\
&LOS Slow&0.100 &0.101 &$\mathbf{1.121}$ &0.082 &0.067 &$\mathbf{1.107}$ &0.049 &0.074 &1.365 &0.201 &0.104 &1.318 \\
&LOS Medium &$\mathbf{0.062}$ &$\mathbf{0.068}$ &1.222 &0.045 &0.062 &1.167 &$\mathbf{0.027}$ &0.057 &$\mathbf{1.360}$ &0.096 &0.084 &$\mathbf{1.280}$ \\
&LOS Fast&$\mathbf{0.062}$ &0.069 &1.123 &$\mathbf{0.044}$ &$\mathbf{0.061}$ &1.160 &$\mathbf{0.027}$ &0.058 &1.535 &$\mathbf{0.094}$ &$\mathbf{0.080}$ &1.282 \\
\cline{2-14}
&JS (Proposed) &$\mathbf{0.062}$ &0.069 &1.131 &0.045 &0.062 &1.160 &$\mathbf{0.027}$ &0.055 &1.521 &$\mathbf{0.094}$ &0.083 &1.301 \\
\cline{2-14}

\multicolumn{1}{c}{\vspace{0.5cm}}\\

\cline{2-14}
\multirow{4}{*}{\textbf{\textbf{Lite}}}
&Depth Loss &1.007 &0.101 &1.716 &0.831 &0.097 &1.835 &0.048 &0.074 &1.789 &1.074  &0.119  &2.011  \\
&LOS Slow&0.090 &0.100 &1.155 &0.138 &0.084 &1.348 &0.049 &0.084 &1.365 &0.304  &0.111  &1.601  \\
&LOS Medium &0.068 &0.076 &$\mathbf{1.154}$ &0.067 &$\mathbf{0.076}$ &$\mathbf{1.141}$ &0.031 &$\mathbf{0.065}$ &$\mathbf{1.265}$ &0.256  &$\mathbf{0.097}$  &1.462  \\
&LOS Fast&0.066 &$\mathbf{0.073}$ &1.208 &0.059 &$\mathbf{0.076}$ &1.182 &$\mathbf{0.030}$ &0.070 &1.309 &0.220  &0.101  &$\mathbf{1.329}$  \\
\cline{2-14}
&JS (Proposed) &$\mathbf{0.064}$ &$\mathbf{0.073}$ &1.280 &$\mathbf{0.056}$ &$\mathbf{0.076}$ &1.373 &$\mathbf{0.030}$ &0.069 &1.281 &$\mathbf{0.166}$ &0.101  &1.411 \\ 
\end{tabular}

\end{table*}

==> tables/loss_comparison_combined.tex <==
\begin{table*}
    \centering
\caption{Map results on loss comparison study. We compare the Depth Loss, LOS at three decay rates, and our propoed JS loss. All numbers are a median of 5 runs.}
\label{tab:loss-comparison}
\begin{tabular}{l l | c c | c c | c c | c c}
&& \multicolumn{2}{c|}{\textbf{Canteen Day}} & \multicolumn{2}{c|}{\textbf{Garden Day}} & \multicolumn{2}{c}{\textbf{MCR Slow 01}}& \multicolumn{2}{c}{\textbf{Quad Easy}} \\
&& $t_{APE}$ & L1 Depth& $t_{APE}$ & L1 Depth& $t_{APE}$ & L1 Depth& $t_{APE}$ & L1 Depth\\
\cline{2-10}
\multirow{4}{*}{\textbf{\textbf{Full}}}
&\textbf{Depth Loss}	&0.887	&2.381	&0.064	&1.149	&0.048	&0.282	&0.189	&0.631 \\
&\textbf{LOS Slow}	  &0.089	&1.127	&\textbf{0.044}	&1.201	&0.046	&0.248	&0.189	&0.384 \\
&\textbf{LOS Medium} &\textbf{0.061}	&1.212	&\textbf{0.044}	&1.167	&\textbf{0.027}	&\textbf{0.178}	&0.094	&0.360 \\
&\textbf{LOS Fast}	  &0.062	&1.508	&0.078	&1.212	&\textbf{0.027}	&0.183	&0.094	&0.384 \\
\cline{2-10}
&\textbf{Proposed}	  &0.062	&\textbf{1.122}	&0.045	&\textbf{1.146}	&\textbf{0.027}	&\textbf{0.178}	&\textbf{0.093}	&\textbf{0.306} \\
\cline{2-10}

\multicolumn{1}{c}{\vspace{0.5cm}}\\
\cline{2-10}
\multirow{4}{*}{\textbf{\textbf{Lite}}}
&\textbf{Depth Loss}	&0.763	&2.776	&0.944	&2.136	&0.045	&0.281	&0.757	&1.137 \\ 
&\textbf{LOS Slow}	  &0.097	&1.762	&0.134	&1.656	&0.045	&0.572	&0.239	&0.780 \\
&\textbf{LOS Medium}	&0.068	&2.089	&0.072	&1.910	&0.031	&1.111	&0.166	&1.313 \\
&\textbf{LOS Fast}	  &0.064	&2.841	&\textbf{0.057}	&2.206	&\textbf{0.029}	&0.497	&0.155	&1.406 \\
\cline{2-10}
&\textbf{Proposed}	  &\textbf{0.063}	&\textbf{1.252}	&\textbf{0.057}	&\textbf{1.321}	&0.030	&\textbf{0.268}	&\textbf{0.137}	&\textbf{0.453} \\
\cline{2-10}
\end{tabular}

\end{table*}

==> tables/loss_comparison_combined_old.tex <==
\begin{table*}
    \centering
\caption{Map results on loss comparison study. All numbers are a median of 5 runs.}
\label{tab:loss-comparison}
\begin{tabular}{l l | c c | c c | c c | c c}
&& \multicolumn{2}{c|}{\textbf{Canteen Day}} & \multicolumn{2}{c|}{\textbf{Garden Day}} & \multicolumn{2}{c}{\textbf{MCR Slow 01}}& \multicolumn{2}{c}{\textbf{Quad Easy}} \\
&& $t_{APE}$ & L1 Depth& $t_{APE}$ & L1 Depth& $t_{APE}$ & L1 Depth& $t_{APE}$ & L1 Depth\\
\cline{2-10}
\multirow{4}{*}{\textbf{\textbf{Full}}}
&Depth Loss&0.160&	1.072&	0.083&	1.328&	0.045&	0.299&	0.303&	0.730 \\
&LOS Slow&0.100&	1.206&	0.082&	1.240&	0.049&	0.254&	0.201&	0.419 \\
&LOS Medium&\textbf{0.062}&	1.300&	0.045&	\textbf{1.162}&	\textbf{0.027}&	0.187&	0.096&	0.360 \\
&LOS Fast&\textbf{0.062}&	1.253&\textbf{0.044}&1.327&	\textbf{0.027}&	0.206&	\textbf{0.094}&	0.410 \\
\cline{2-10}
&Proposed&\textbf{0.062}&	\textbf{1.054}&	0.045&	1.166&	\textbf{0.027}&	\textbf{0.183}&	\textbf{0.094}&	\textbf{0.339} \\
\cline{2-10}

\multicolumn{1}{c}{\vspace{0.5cm}}\\
\cline{2-10}
\multirow{4}{*}{\textbf{\textbf{Lite}}}
&Depth Loss&1.007&	3.099&	0.831&	2.095&	0.048&	0.291&	1.074&	1.358 \\
&LOS Slow&0.090&	1.758&	0.138&	1.614&	0.049&	0.583&	0.304&	1.034 \\
&LOS Medium&0.068&	2.325&	0.067&	1.984&	0.031&	1.141&	0.256&	1.707 \\
&LOS Fast&0.066&	2.552&	0.059&	2.198&	\textbf{0.030}&	0.536&	0.220&	1.792 \\
\cline{2-10}
&Proposed&\textbf{0.064}&	\textbf{1.356}&	\textbf{0.056}&	\textbf{1.335}&	\textbf{0.030}&\textbf{0.275}&	\textbf{0.166}&	\textbf{0.472} \\
\cline{2-10}
\end{tabular}

\end{table*}

==> tables/loss_comparison_compact.tex <==
\begin{table*}
    \centering
\caption{Map results on loss comparison study. All numbers are a median of 5 runs.}
\label{loss-comparison-map-compact}
\begin{tabular}{l l | c c | c c | c c | c c}
&& \multicolumn{2}{c|}{\textbf{Canteen Day}} & \multicolumn{2}{c|}{\textbf{Garden Day}} & \multicolumn{2}{c}{\textbf{MCR Slow 01}}& \multicolumn{2}{c}{\textbf{Quad Easy}} \\
&& Acc. & Comp. & Acc. & Comp. & Acc. & Comp. & Acc. & Comp. \\
\cline{2-10}
\multirow{4}{*}{\textbf{\textbf{Full}}}
&Depth Loss&0.647  &0.155  &0.267  &0.473  &0.068  &0.170  &1.004  &0.864  \\
&LOS Slow&0.524  &0.136  &0.157  &0.565  &0.041  &0.086  &0.293  &0.387  \\
&LOS Medium&0.405  &0.119  &0.182  &0.255  &0.046  &0.054  &0.160  &0.403  \\
&LOS Fast&0.401  &0.127  &0.198  &0.317  &0.048  &0.055  &0.193  &0.407  \\
\cline{2-10}
Proposed&0.926  &0.083  &0.201  &0.251  &0.047  &0.054  &0.346  &0.295  \\
\cline{2-10}

\multicolumn{1}{c}{\vspace{0.5cm}}\\
\cline{2-10}
\multirow{4}{*}{\textbf{\textbf{Lite}}}
&Depth Loss&0.508  &1.564  &0.305  &2.816  &0.041  &0.781  &0.630  &1.152  \\
&LOS Slow&0.575  &0.436  &0.147  &0.774  &0.084  &0.341  &0.457  &0.844  \\
&LOS Medium&0.379  &0.345  &0.217  &0.694  &0.116  &0.168  &0.511  &0.787  \\
&LOS Fast&0.326  &0.380  &0.150  &0.911  &0.094  &0.111  &0.452  &0.717  \\
\cline{2-10}
&Proposed&0.665  &0.227  &0.138  &0.509  &0.042  &0.100  &0.509  &0.776  \\
\cline{2-10}
\end{tabular}

\end{table*}

==> tables/loss_comparison_map.tex <==
\begin{sidewaystable*}
    \centering
\caption{Map results on loss comparison study. All numbers are a median of 5 runs.}
\label{loss-comparison-map}
\begin{tabular}{l l | c c c c |c c c c |c c c c |c c c c}
&& \multicolumn{4}{c|}{\textbf{Canteen Day}} & \multicolumn{4}{c|}{\textbf{Garden Day}} & \multicolumn{4}{c}{\textbf{MCR Slow 01}}& \multicolumn{4}{c}{\textbf{Quad Easy}} \\
&& Acc. & Comp. & Precision & Recall & Acc. & Comp. & Precision & Recall & Acc. & Comp. & Precision & Recall & Acc. & Comp. & Precision & Recall \\
\cline{2-18}
\multirow{4}{*}{\textbf{\textbf{Full}}}
&Depth Loss&0.750  &0.149  &0.351  &0.889  &0.244  &0.576  &0.420  &0.669  &0.068  &0.139  &0.796  &0.954  &1.091  &0.778  &0.118  &0.464  \\
&LOS Slow&0.448  &0.140  &0.454  &0.900  &0.152  &0.654  &0.635  &0.785  &0.040  &0.117  &0.938  &0.971  &0.200  &0.387  &0.472  &0.887  \\
&LOS Medium&0.405  &0.119  &0.486  &0.944  &0.203  &0.250  &0.655  &0.873  &0.049  &0.054  &0.897  &0.980  &0.160  &0.404  &0.648  &0.912  \\
&LOS Fast&0.401  &0.128  &0.489  &0.945  &0.214  &0.317  &0.654  &0.863  &0.049  &0.052  &0.893  &0.980  &0.192  &0.356  &0.657  &0.921  \\
\cline{2-18}
&Proposed&0.855  &0.083  &0.458  &0.938  &0.201  &0.251  &0.623  &0.834  &0.047  &0.055  &0.910  &0.978  &0.296  &0.265  &0.653  &0.917  \\
\cline{2-18}

\multicolumn{1}{c}{\vspace{0.5cm}}\\
\cline{2-18}
\multirow{4}{*}{\textbf{\textbf{Lite}}}
&Depth Loss&0.515  &1.254  &0.201  &0.291  &0.225  &2.196  &0.378  &0.349  &0.040  &0.781  &0.931  &0.893  &0.681  &1.075  &0.165  &0.478  \\
&LOS Slow&0.653  &0.453  &0.424  &0.708  &0.141  &0.773  &0.586  &0.651  &0.080  &0.348  &0.721  &0.884  &0.484  &0.879  &0.175  &0.579  \\
&LOS Medium&0.381  &0.337  &0.383  &0.843  &0.223  &0.694  &0.430  &0.706  &0.116  &0.159  &0.618  &0.938  &0.432  &0.712  &0.246  &0.748  \\
&LOS Fast&0.334  &0.377  &0.496  &0.874  &0.151  &0.924  &0.638  &0.730  &0.094  &0.109  &0.731  &0.965  &0.342  &0.618  &0.283  &0.672  \\
\cline{2-18}
&Proposed&0.690  &0.222  &0.519  &0.877  &0.141  &0.503  &0.699  &0.756  &0.044  &0.098  &0.901  &0.966  &0.472  &0.692  &0.233  &0.542  \\
\cline{2-18}
\end{tabular}

\end{sidewaystable*}


==> tables/map_comparison.tex <==
\begin{table}
  \centering
  \caption{Comparison of map Acccuracy, Completion, Precision, and Recall between proposed and baseline algorithms. All numbers are a median of five runs.}
  \label{tab:map-comparison}
  \begin{tabular}{l l | c c c | c c}
  && \textbf{LeGO} & \textbf{LIO} & \textbf{NICE} & \multirow{2}{*}{\textbf{\algname}} & \textbf{\algname}\\
  && \textbf{LOAM} & \textbf{SAM} & \textbf{SLAM} & &\textbf{lite}  \\
    \hline
    \multirow{4}{*}{\verttab{\textbf{Canteen}}}
    &Acc. $\downarrow$ & 0.678& 2.129& \fail& 0.454& 0\textbf{.451} \\
    &Comp. $\downarrow$& 0.082& \textbf{0.060}& \fail& 0.173& 0.190 \\
    &Prec. $\uparrow$ & \textbf{0.624}& 0.494& \fail& 0.335& 0.274 \\
    &Rec.  $\uparrow$ & 0.846& 0.901& \fail& \textbf{0.902}& 0.870 \\
    \hline
    \multirow{4}{*}{\verttab{\textbf{Garden}}}
    &Acc. $\downarrow$ & \textbf{0.157}& 0.283& \fail& 0.277& 0.271 \\
    &Comp. $\downarrow$& 0.100&\textbf{ 0.063}& \fail& 0.170& 0.232 \\
    &Prec. $\uparrow$ & \textbf{0.786}& 0.739& \fail& 0.456& 0.379 \\
    &Rec.  $\uparrow$ & 0.778& \textbf{0.858}& \fail& 0.799& 0.750 \\
    \hline
    \multirow{4}{*}{\verttab{\textbf{MCR}}}
    &Acc. $\downarrow$ & \textbf{0.055}& 0.110& 0.621& 0.132& 0.131 \\
    &Comp. $\downarrow$& 0.149& \textbf{0.045}& 0.419& 0.079& 0.100 \\
    &Prec. $\uparrow$ & \textbf{0.916}& 0.805& 0.124& 0.675& 0.603 \\
    &Rec.  $\uparrow$ & 0.073& 0.676& 0.476& \textbf{0.954}& 0.928 \\
    \hline
    \multirow{4}{*}{\verttab{\textbf{Quad}}}
    &Acc. $\downarrow$ & \textbf{0.062}& 0.116& \fail& 0.335& 0.550 \\
    &Comp. $\downarrow$& 0.133& \textbf{0.065}& \fail& 0.381& 0.659 \\
    &Prec. $\uparrow$ & \textbf{0.877}& 0.650& \fail& 0.443& 0.187 \\
    &Rec.  $\uparrow$ & 0.605& \textbf{0.902}& \fail& 0.895& 0.623 \\
  \end{tabular}
\end{table}

==> tables/map_comparison_old.tex <==
\begin{table}
  \centering
  \caption{Comparison of map Acc. $\downarrow$ between proposed and baseline algorithms. All numbers are a median of five runs.}
  \label{tab:map-comparison}
  \begin{tabular}{l l | c c c | c c}
  && \textbf{LeGO} & \textbf{LIO} & \textbf{NICE} & \multirow{2}{*}{\textbf{\algname}} & \textbf{\algname}\\
  && \textbf{LOAM} & \textbf{SAM} & \textbf{SLAM} & &\textbf{lite}  \\
  \hline
  \multirow{4}{*}{\verttab{\textbf{Canteen}}}
      &Acc. $\downarrow$&0.677&	2.130&	\fail&	0.926&	\textbf{0.665} \\
      &Comp. $\downarrow$&0.082&	\textbf{0.060}&	\fail&	0.083&	0.227 \\
      &Prec. $\uparrow$&\textbf{0.624}&	0.494&	\fail&	0.458&	0.519 \\
      &Rec. $\uparrow$&0.846&	0.900&	\fail&	\textbf{0.939}&	0.875 \\
  \hline
  \multirow{4}{*}{\verttab{\textbf{Garden}}}
      &Acc. $\downarrow$&0.157&	0.283&	\fail&	0.201&	\textbf{0.138}\\
      &Comp. $\downarrow$&0.100&	\textbf{0.063}&	\fail&	0.251&	0.509 \\
      &Prec. $\uparrow$&\textbf{0.786}&	0.739&	\fail&	0.623&	0.696 \\
      &Rec. $\uparrow$&0.778&	\textbf{0.858}&	\fail&	0.841&	0.748 \\
  \hline
  \multirow{4}{*}{\verttab{\textbf{MCR}}}
      &Acc. $\downarrow$&0.055&	0.110&	0.626&	0.047&	\textbf{0.042} \\
      &Comp. $\downarrow$&0.149&	\textbf{0.045}&	0.435&	0.054&	0.100 \\
      &Prec. $\uparrow$&\textbf{0.917}&	0.805&	0.120&	0.906&	0.914 \\
      &Rec. $\uparrow$&0.073&	0.675&	0.464&	\textbf{0.978}&	0.966 \\
  \hline
  \multirow{4}{*}{\verttab{\textbf{Quad}}}
      &Acc. $\downarrow$&\textbf{0.062}&	0.116&	\fail&	0.346&	0.509 \\
      &Comp. $\downarrow$&0.133&	\textbf{0.065}&	\fail&	0.295&	0.776 \\
      &Prec. $\uparrow$ &\textbf{0.877}&	0.650&	\fail&	0.615&	0.187 \\
      &Rec. $\uparrow$&0.605&	0.902&	\fail&	\textbf{0.911}&	0.479 \\
  \end{tabular}
\end{table}


% \begin{sidewaystable*}[]\label{tab:map-comparison}
%     \centering
% \begin{tabular}{l | c c c c |c c c c |c c c c |c c c c}
% & \multicolumn{4}{c|}{\textbf{Canteen Day}} & \multicolumn{4}{c|}{\textbf{Garden Day}} & \multicolumn{4}{c}{\textbf{MCR Slow 01}}& \multicolumn{4}{c}{\textbf{Quad Easy}} \\
% & Acc. & Comp. & Prec. & Rec. & Acc. & Comp. & Prec. & Rec. & Acc. & Comp. & Prec. & Rec. & Acc. & Comp. & Prec. & Rec. \\
% \hline
% Lego-LOAM&\fail  &0.081  &0.624  &0.854  &0.144  &0.098  &0.808  &0.779  &0.054  &0.114  &0.918  &0.081  &0.062  &0.133  &0.877  &0.605  \\
% LIO-SAM&\fail  &0.060  &0.494  &0.899  &0.270  &0.066  &0.751  &0.838  &0.110  &0.045  &0.805  &0.675  &0.087  &0.051  &0.760  &0.973  \\
% NICE-SLAM & \fail & \fail & \fail & \fail & \fail & \fail & \fail & \fail & 0.552  &0.441  &0.131  &0.464 & \fail & \fail & \fail & \fail \\
% \hline
% \algname&\fail  &0.083  &0.458  &0.938  &0.201  &0.251  &0.623  &0.834  &0.047  &0.055  &0.910  &0.978  &0.296  &0.265  &0.653  &0.917  \\
% \algname lite&\fail  &0.222  &0.519  &0.877  &0.141  &0.503  &0.699  &0.756  &0.044  &0.098  &0.901  &0.966  &0.472  &0.692  &0.233  &0.542  \\
% \end{tabular}
% \end{sidewaystable*}

==> tables/reconstruction_results.tex <==
\begin{table}[h] 
\begin{center}
\caption{Map Reconstruction Results on Fusion Portable, evaluated on the MCR Sequence}
\label{reconstruction}
\begin{tabular}{l c c c c}
\hline
& \multirow{2}{*}{\textbf{Depth L1} $\downarrow$} & \multirow{2}{*}{\textbf{Acc.} $\downarrow$} & \multirow{2}{*}{\textbf{Comp.\ } $\downarrow$} & \textbf{Comp.}\\
&&&& \textbf{Ratio} $\uparrow$ \\
\hline
\textbf{NICE-SLAM} & 0 & 0 & 0 & 0 \\
\textbf{iMAP$^*$} & 0 & 0 & 0 & 0 \\
\textbf{\algname} & 0 & 0 & 0 & 0\\
\textbf{\algname lite} & 0 & 0 & 0 & 0\\
\hline
\end{tabular}  
\end{center}
\end{table}

==> tables/runtime.tex <==
\begin{table} 
\begin{center}
\caption{Runtime statistics for tracking a single Frame mapping, a single KeyFrame, and average time per KeyFrame to run both in parallel.}
 \label{tab:runtime}
\begin{tabular}{l c c c}
\hline
& \multirow{2}{*}{\textbf{Tracking (s)}} & \multirow{2}{*}{\textbf{Mapping (s)}} & \textbf{Avg. Per} \\
& & & \textbf{KeyFrame (s)}\\
\hline
\textbf{\algname}& 0.024 & 15.04 & 15.17\\
\textbf{\algname lite} & 0.013 & 2.34 & 2.79 \\
\hline
\end{tabular}   
\end{center}
\end{table}

==> tables/tracking_comparison.tex <==
\begin{table*}  
\begin{center}
\caption{Pose tracking results on Fusion Portable sequences. $t_{ATE}$ is RMSE ATE (m), $t_{rel}$ is RMSE 3m relative translation error, and $r_{rel}$ is RMSE 3m relative rotation error (deg). All numbers are a median of 5 runs.}
\label{tab:tracking-comparison}
\begin{tabular}{l | c c c | c c c | c c c | c c c}
& \multicolumn{3}{c|}{\textbf{Canteen Day}} & \multicolumn{3}{c|}{\textbf{Garden Day}} & \multicolumn{3}{c}{\textbf{MCR Slow 01}} & \multicolumn{3}{c}{\textbf{Quad Easy}} \\
& $t_{ATE}$ & $t_{rel}$ & $r_{rel}$ & $t_{ATE}$ & $t_{rel}$ & $r_{rel}$ & $t_{ATE}$ & $t_{rel}$ & $r_{rel}$& $t_{ATE}$ & $t_{rel}$ & $r_{rel}$\\
\hline
\textbf{LeGO-LOAM}&0.129  &0.228  &4.104  &0.161  &0.361  &5.488  &0.052  &0.084  &4.503  &0.126  &0.188  &2.966  \\
\textbf{LIO-SAM}&0.084  &0.076  &\textbf{0.415}  &\textbf{0.042}  &\textbf{0.044} &\textbf{0.467}  &\textbf{0.026}  &0.059  &\textbf{1.501}  &\textbf{0.080}  &0.089  &1.396  \\
\textbf{NICE-SLAM} & \fail & \fail & \fail & \fail & \fail & \fail & 0.248  &0.222  &3.921 & \fail & \fail & \fail \\
\hline
\textbf{\algname} & \textbf{0.062}  &\textbf{0.070}  &1.269  &0.045  &0.061  &1.174  &0.027  &\textbf{0.056}  &1.554  &0.093  &\textbf{0.080}  &\textbf{1.172}  \\
\textbf{\algname lite} &0.063  &0.077  &1.186  &0.057  &0.076  &1.343  &0.030  &0.070  &1.277  &0.137  &0.092  &1.240  \\
\hline
\end{tabular}
\end{center}
\end{table*}

==> tables/traj_ablation.tex <==
\begin{table*}
    \centering
\caption{Trajectory tracking results on SLAM ablation study. $t_{ATE}$ is RMS ATE (m), $t_{rel}$ is RMS 3m relative translation error, and $r_{rel}$ is RMS 3m relative rotation error (deg). All numbers are a median of 5 runs.}
 \label{tab:traj-ablation}
\begin{tabular}{l l | c c c | c c c | c c c | c c c}
&& \multicolumn{3}{c|}{\textbf{Canteen Day}} & \multicolumn{3}{c|}{\textbf{Garden Day}} & \multicolumn{3}{c}{\textbf{MCR Slow 01}}& \multicolumn{3}{c}{\textbf{Quad Easy}}  \\
&& $t_{ATE}$ & $t_{rel}$ & $r_{rel}$ & $t_{ATE}$ & $t_{rel}$ & $r_{rel}$ & $t_{ATE}$ & $t_{rel}$ & $r_{rel}$& $t_{ATE}$ & $t_{rel}$ & $r_{rel}$\\
\cline{2-14}
\multirow{5}{*}{\textbf{\textbf{Full}}}
&No Pose Opt. &1.060 &$\mathbf{0.067}$ &1.317 &1.256 &0.064 &1.273 &0.081 &0.065 &1.605 &0.583  &$\mathbf{0.079}$  &1.267  \\
&No Motion Comp. &0.065 &0.075 &1.183 &0.047 &0.061 &$\mathbf{1.102}$ &0.028 &0.054 &1.375 &0.097  &0.087  &1.205  \\
&Random KFs &$\mathbf{0.062}$ &$\mathbf{0.067}$ &1.226 &$\mathbf{0.045}$ &$\mathbf{0.060}$ &1.162 &$\mathbf{0.027}$ &$\mathbf{0.051}$ &$\mathbf{1.278}$ &$\mathbf{0.091}$  &0.083  &1.231  \\
&Recent KFs &$\mathbf{0.062}$ &$\mathbf{0.067}$ &1.286 &0.047 &0.062 &1.161 &$\mathbf{0.027}$ &0.061 &1.548 &0.254  &0.083  &$\mathbf{1.193}$  \\
\cline{2-14}
&Proposed &$\mathbf{0.062}$ &0.069 &$\mathbf{1.131}$ &$\mathbf{0.045}$ &0.062 &1.160 &$\mathbf{0.027}$ &0.055 &1.521 &0.094  &0.083  &1.301  \\
\cline{2-14}
\multicolumn{1}{c}{\vspace{0.5cm}}\\
\cline{2-14}
\multirow{5}{*}{\textbf{\textbf{Lite}}}
&Pose Opt. &1.083 &$\mathbf{0.069}$ &$\mathbf{1.265}$ &1.119 &$\mathbf{0.061}$ &1.338 &0.088 &0.060 &1.535 &0.903  &0.084  &1.253  \\
&No Motion Comp. &0.065 &0.075 &1.280 &0.062 &0.074 &1.352 &$\mathbf{0.030}$ &$\mathbf{0.057}$ &1.600 &0.433  &0.100  &1.387  \\
&Random KFs &$\mathbf{0.063}$ &0.073 &1.160 &0.058 &0.074 &$\mathbf{1.151}$ &$\mathbf{0.030}$ &0.070 &1.288 &$\mathbf{0.129}$  &0.090  &1.290  \\
&Recent KFs &0.087 &0.071 &1.259 &0.074 &0.073 &1.184 &$\mathbf{0.030}$ &0.069 &$\mathbf{1.274}$ &0.265  &$\mathbf{0.089}$  &$\mathbf{1.288}$  \\
\cline{2-14}
&Proposed &0.064 &0.073 &1.280 &$\mathbf{0.056}$ &0.076 &1.373 &$\mathbf{0.030}$ &0.069 &1.281 &0.166  &0.101  &1.411  \\
\cline{2-14}
\end{tabular}
\end{table*}

==> tables/traj_ablation_combined.tex <==
\begin{table*}
\centering
\caption{Results of SLAM ablation study in the full and lite configurations. In the first row, pose optimization is enabled. In the next three rows we compare the impact of KeyFrame selection being fully deterministic, hybrid, and fully random. All numbers are a median of five runs.}
\label{tab:traj-ablation}
\begin{tabular}{l c c | c c | c c | c c | c c}
&\multicolumn{2}{c|}{\textbf{Configuration}}& \multicolumn{2}{c|}{\textbf{Canteen Day}} & \multicolumn{2}{c|}{\textbf{Garden Day}} & \multicolumn{2}{c}{\textbf{MCR Slow 01}}& \multicolumn{2}{c}{\textbf{Quad Easy}} \\

&Pose&Rand&$t_{APE}$ & L1 Depth& $t_{APE}$ & L1 Depth& $t_{APE}$ & L1 Depth& $t_{APE}$ & L1 Depth\\
\cline{2-11}
\multirow{4}{*}{\textbf{\textbf{Full}}}
& \emptycirc & \fullcirc  & 1.060& 3.125& 1.256& 2.778& 0.081& 0.282& 0.579& 1.177 \\
& \fullcirc &  \emptycirc & \textbf{0.062}& 1.373& 0.047& 1.316& 0.027& 0.206& 0.307& 0.967 \\
& \fullcirc &  \halfcirc  & \textbf{0.062}& \textbf{1.076}& \textbf{0.045}& \textbf{1.124}& \textbf{0.027}& \textbf{0.175}& 0.095& 0.336 \\
\cline{2-11}
& \fullcirc & \fullcirc  & \textbf{0.062}& 1.122& \textbf{0.045}& 1.146& \textbf{0.027}& 0.178& \textbf{0.093}&\textbf{0.306} \\
\cline{2-11}

\multicolumn{1}{c}{\vspace{0.5cm}}\\
\cline{2-11}
\multirow{4}{*}{\textbf{\textbf{Lite}}}
& \emptycirc & \fullcirc  & 1.083& 3.682& 1.120& 3.444& 0.088& 0.306& 0.897& 1.615 \\
& \fullcirc &  \emptycirc & 0.078& 1.667& 0.075& 1.379& \textbf{0.030}& \textbf{0.258}& 0.279& 0.818 \\
& \fullcirc &  \halfcirc  & 0.064& 1.342& 0.060& \textbf{1.220}&\textbf{0.030}& 0.281& 0.151& 0.467 \\
\cline{2-11}
& \fullcirc & \fullcirc  & \textbf{0.063}& \textbf{1.252}& \textbf{0.057}& 1.321& \textbf{0.030}& 0.268& \textbf{0.137}& \textbf{0.453} \\
\cline{2-11}
\end{tabular}

\end{table*}

==> tables/traj_ablation_combined_old.tex <==
\begin{table*}
\centering
\caption{Map results on loss comparison study. All numbers are a median of 5 runs.}
\label{tab:traj-ablation}
\begin{tabular}{l | c c c | c c | c c | c c | c c | c c}
&\multicolumn{3}{c|}{\textbf{Configuration}}& \multicolumn{2}{c|}{\textbf{Canteen Day}} & \multicolumn{2}{c|}{\textbf{Garden Day}} & \multicolumn{2}{c}{\textbf{MCR Slow 01}}& \multicolumn{2}{c}{\textbf{Quad Easy}} \\
&Pose&Rand&Motion& $t_{APE}$ & L1 Depth& $t_{APE}$ & L1 Depth& $t_{APE}$ & L1 Depth& $t_{APE}$ & L1 Depth\\
\cline{2-12}
\multirow{4}{*}{\textbf{\textbf{Full}}}
& \emptycirc & \halfcirc  & \fullcirc &  1.060&	3.402&	1.256&	3.205&	0.081&	0.384&	0.583&	1.430 \\
& \fullcirc & \halfcirc  & \emptycirc &  0.065&	1.078&	0.047&	1.172&	0.028&	0.177&	0.097&	\textbf{0.325} \\
& \fullcirc & \fullcirc  & \fullcirc & \textbf{0.062}&	\textbf{0.974}&	\textbf{0.045}&	\textbf{1.131}&	\textbf{0.027}&	\textbf{0.183}&	\textbf{0.091}&	0.359 \\
& \fullcirc & \emptycirc  & \fullcirc &  \textbf{0.062}&	1.253&	0.047&	1.380&	\textbf{0.027}&	0.211&	0.254&	0.749 \\
\cline{2-12}
& \fullcirc & \halfcirc  & \fullcirc & \textbf{0.062}&	1.054&	\textbf{0.045}&	1.166&	\textbf{0.027}&	\textbf{0.183}&	0.094&	0.339 \\
\cline{2-12}

\multicolumn{1}{c}{\vspace{0.5cm}}\\
\cline{2-12}
\multirow{4}{*}{\textbf{\textbf{Lite}}}
& \emptycirc & \halfcirc  & \fullcirc  &  1.083&	5.533&	1.119&	3.960&	0.088&	0.535&	0.903&	1.853 \\
& \fullcirc & \halfcirc  & \emptycirc &  0.065&	\textbf{1.251}&	0.062&	1.384&	\textbf{0.030}&	0.262&	0.433&	1.023 \\
& \fullcirc & \fullcirc  & \fullcirc & \textbf{0.063}&	1.412&	0.058&	1.345&	\textbf{0.030}&	0.259&	\textbf{0.129}&	\textbf{0.468} \\
& \fullcirc & \emptycirc  & \fullcirc & 0.087&	1.748&	0.074&	1.451&	\textbf{0.030}&	\textbf{0.252}&	0.265&	0.921 \\
\cline{2-12}
& \fullcirc & \halfcirc  & \fullcirc & 0.064&	1.356&	\textbf{0.056}&	\textbf{1.335}&	\textbf{0.030}&	0.275&	0.166&	0.472 \\
\cline{2-12}
\end{tabular}

\end{table*}

==> tables/traj_ablation_compact.tex <==
\begin{table}
    \centering
    \label{tab:traj-ablation-compact}
\begin{tabular}{l l | c c c c}
&& \textbf{Canteen} & \textbf{Garden} & \textbf{MCR} & \textbf{Quad}  \\
\cline{2-6}
\multirow{5}{*}{\textbf{\textbf{Full}}}
&No Pose Opt.&1.060  &1.256  &0.081  &0.583  \\
&No Motion Comp.&0.065  &0.047  &0.028  &0.097  \\
&Random KFs&0.062  &0.045  &0.027  &0.091  \\
&Temporal KFs&0.062  &0.047  &0.027  &0.254  \\
\cline{2-6}
&Proposed&0.062  &0.045  &0.027  &0.094  \\
\cline{2-6}
\multicolumn{1}{c}{\vspace{0.5cm}}\\
\cline{2-6}
\multirow{5}{*}{\textbf{\textbf{Lite}}}
&No Pose Opt.&1.083  &1.119  &0.088  &0.903  \\
&No Motion Comp.&0.065  &0.062  &0.030  &0.433  \\
&Random KFs&0.063  &0.058  &0.030  &0.129  \\
&Temporal KFs&0.087  &0.074  &0.030  &0.265  \\
\cline{2-6}
&Proposed&0.064  &0.056  &0.030  &0.166  \\
\cline{2-6}
\end{tabular}
\end{table}

==> tables/traj_ablation_map.tex <==

\begin{sidewaystable*}
    \centering
\caption{Map results on loss comparison study. All numbers are a median of 5 runs.}
\label{traj-comparison-map}
\begin{tabular}{l l | c c c c |c c c c |c c c c |c c c c}
&& \multicolumn{4}{c|}{\textbf{Canteen Day}} & \multicolumn{4}{c|}{\textbf{Garden Day}} & \multicolumn{4}{c}{\textbf{MCR Slow 01}}& \multicolumn{4}{c}{\textbf{Quad Easy}} \\
&& Acc. & Comp. & Precision & Recall & Acc. & Comp. & Precision & Recall & Acc. & Comp. & Precision & Recall & Acc. & Comp. & Precision & Recall \\
\cline{2-18}
\multirow{4}{*}{\textbf{\textbf{Full}}}
&No Pose Opt.&0.721  &0.668  &0.187  &0.540  &0.820  &1.108  &0.134  &0.242  &0.067  &0.168  &0.810  &0.948  &0.855  &0.924  &0.124  &0.383  \\
&No Mo. Comp.&0.388  &0.101  &0.462  &0.930  &0.201  &0.284  &0.625  &0.840  &0.049  &0.058  &0.897  &0.976  &0.433  &0.280  &0.600  &0.909  \\
&Random KFs&0.404  &0.085  &0.475  &0.940  &0.198  &0.253  &0.641  &0.847  &0.048  &0.059  &0.899  &0.978  &0.438  &0.266  &0.629  &0.926  \\
&Temporal KFs&0.399  &0.166  &0.394  &0.883  &0.204  &0.264  &0.569  &0.798  &0.046  &0.065  &0.903  &0.976  &0.646  &0.691  &0.118  &0.347  \\
\cline{2-18}
&Proposed&0.855  &0.083  &0.458  &0.938  &0.201  &0.251  &0.623  &0.834  &0.047  &0.055  &0.910  &0.978  &0.296  &0.265  &0.653  &0.917  \\
\cline{2-18}

\multicolumn{1}{c}{\vspace{0.5cm}}\\
\cline{2-18}
\multirow{4}{*}{\textbf{\textbf{Lite}}}
&No Pose Opt.&0.900  &1.212  &0.085  &0.197  &0.811  &1.479  &0.131  &0.173  &0.060  &0.251  &0.858  &0.939  &0.731  &1.286  &0.138  &0.410  \\
&No Mo. Comp.&0.567  &0.235  &0.523  &0.870  &0.135  &0.528  &0.684  &0.740  &0.042  &0.104  &0.912  &0.966  &0.694  &1.108  &0.118  &0.354  \\
&Random KFs&0.625  &0.215  &0.526  &0.869  &0.149  &0.507  &0.695  &0.762  &0.045  &0.103  &0.898  &0.966  &0.407  &0.666  &0.266  &0.597  \\
&Temporal KFs&0.631  &0.233  &0.498  &0.849  &0.145  &0.530  &0.671  &0.728  &0.044  &0.100  &0.909  &0.968  &0.763  &1.017  &0.098  &0.293  \\
\cline{2-18}
&Proposed&0.690  &0.222  &0.519  &0.877  &0.141  &0.503  &0.699  &0.756  &0.044  &0.098  &0.901  &0.966  &0.472  &0.692  &0.233  &0.542  \\
\cline{2-18}
\end{tabular}

\end{sidewaystable*}

==> tables/traj_ablation_map_compact.tex <==
\begin{table*}[]
    \centering
\caption{Map results on SLAM comparison study. All numbers are a median of 5 runs.}
\label{tab:traj-comparison-map-compact}
\begin{tabular}{l l | c c | c c | c c | c c}
&& \multicolumn{2}{c|}{\textbf{Canteen Day}} & \multicolumn{2}{c|}{\textbf{Garden Day}} & \multicolumn{2}{c}{\textbf{MCR Slow 01}}& \multicolumn{2}{c}{\textbf{Quad Easy}} \\
&& Acc. & Comp. & Acc. & Comp. & Acc. & Comp. & Acc. & Comp. \\
\cline{2-10}
\multirow{4}{*}{\textbf{\textbf{Full}}}
&No Pose Opt.&0.732  &0.697  &0.830  &1.117  &0.071  &0.142  &0.758  &1.107  \\
&No Motion Comp.&0.918  &0.094  &0.205  &0.272  &0.047  &0.058  &0.425  &0.290  \\
&Random KFs&0.412  &0.088  &0.202  &0.253  &0.048  &0.059  &0.344  &0.285  \\
&Temporal KFs&0.402  &0.148  &0.210  &0.289  &0.047  &0.059  &0.622  &0.679  \\
\cline{2-10}
&Proposed&0.926  &0.083  &0.201  &0.251  &0.047  &0.054  &0.346  &0.295  \\
\cline{2-10}

\multicolumn{1}{c}{\vspace{0.5cm}}\\
\cline{2-10}
\multirow{4}{*}{\textbf{\textbf{Lite}}}
&No Pose Opt.&0.816  &1.245  &0.804  &1.499  &0.060  &0.234  &0.807  &1.196  \\
&No Motion Comp.&0.555  &0.244  &0.135  &0.550  &0.044  &0.108  &0.694  &1.108  \\
&Random KFs&0.622  &0.233  &0.145  &0.507  &0.045  &0.103  &0.427  &0.666  \\
&Temporal KFs&0.577  &0.258  &0.145  &0.528  &0.045  &0.102  &0.752  &0.999  \\
\cline{2-10}
&Proposed&0.665  &0.227  &0.138  &0.509  &0.042  &0.100  &0.509  &0.776  \\
\cline{2-10}
\end{tabular}
\end{table*}
